Evaluating the Robustness of Retrieval Pipelines with Query Variation Generators

Heavily pre-trained transformers for language modelling, such as BERT, have shown to be remarkably effective for Information Retrieval (IR) tasks, typically applied to re-rank the results of a first-stage retrieval model. IR benchmarks evaluate the effectiveness of retrieval pipelines based on the premise that a single query is used to instantiate the underlying information need. However, previous research has shown that (I) queries generated by users for a fixed information need are extremely variable and, in particular, (II) neural models are brittle and often make mistakes when tested with modified inputs. Motivated by those observations we aim to answer the following question: how robust are retrieval pipelines with respect to different variations in queries that do not change the queries' semantics? In order to obtain queries that are representative of users' querying variability, we first created a taxonomy based on the manual annotation of transformations occurring in a dataset (UQV100) of user-created query variations. For each syntax-changing category of our taxonomy, we employed different automatic methods that when applied to a query generate a query variation. Our experimental results across two datasets for two IR tasks reveal that retrieval pipelines are not robust to these query variations, with effectiveness drops of $\approx20\%$ on average. The code and datasets are available at https://github.com/Guzpenha/query_variation_generators.

==> tables/main_table_antique.tex <==
% \begin{table*}[ht!]
% \caption{Effectiveness (nDCG@10) of different methods for \antique{} when faced with different query variations. Bold indicates the highest values observed for each model and ${\downarrow}/{\uparrow}$ subscripts indicate statistically significant losses/improvements, using two-sided paired Student's T-Test at 95\% confidence interval when compared against the same model with the original queries. $\# q$ indicates the number of valid query variations for the method (invalid query variations are replaced by the original query).}
% \label{table:main_table_antique}

% \begin{tabular}{@{}lllllllllr@{}}
% \toprule
%  &  & \multicolumn{7}{c}{\antique{}} & \multicolumn{1}{l}{} \\ \midrule
% Category & Query Variation & \bm{} & \bmrm{} & \KNRM{} & \CKNRM{} & \EPIC{} & \BERT{} & \T{} & \multicolumn{1}{l}{\# q} \\ \midrule
% - & original query & \textbf{0.2286} & \textbf{0.2169} & 0.2175 & 0.2065 & 0.2663 & \textbf{0.4212} & \textbf{0.3338} & 200 \\  \hdashline
% \multirow{3}{*}{\misspelling{}} & \charswap{} & 0.1559$^{\downarrow}$ & 0.1478$^{\downarrow}$ & 0.1590$^{\downarrow}$ & 0.1451$^{\downarrow}$ & 0.1841$^{\downarrow}$ & 0.2868$^{\downarrow}$ & 0.2514$^{\downarrow}$ & 199 \\ 
%  & \charsub{} & 0.1623$^{\downarrow}$ & 0.1593$^{\downarrow}$ & 0.1558$^{\downarrow}$ & 0.1476$^{\downarrow}$ & 0.1887$^{\downarrow}$ & 0.2797$^{\downarrow}$ & 0.2486$^{\downarrow}$ & 182 \\
%  & \charqwerty{} & 0.1613$^{\downarrow}$ & 0.1527$^{\downarrow}$ & 0.1602$^{\downarrow}$ & 0.1550$^{\downarrow}$ & 0.1922$^{\downarrow}$ & 0.2987$^{\downarrow}$ & 0.2664$^{\downarrow}$ & 197 \\ \midrule
% \multirow{2}{*}{\naturality{}} & \removestop{} & 0.2270 & 0.2160 & \textbf{0.2222} & \textbf{0.2153} & \textbf{0.2693} & 0.3830$^{\downarrow}$ & 0.3200$^{\downarrow}$ & 199 \\
%  & \tfiverectotitle{} & 0.1673$^{\downarrow}$ & 0.1646$^{\downarrow}$ & 0.1601$^{\downarrow}$ & 0.1669$^{\downarrow}$ & 0.2000$^{\downarrow}$ & 0.2695$^{\downarrow}$ & 0.2397$^{\downarrow}$ & 136 \\ \midrule
% \ordering{} & \orderswap{} & 0.2286 & 0.2168 & 0.2178 & 0.1978$^{\downarrow}$ & 0.2665 & 0.4134$^{\downarrow}$ & 0.3248$^{\downarrow}$ & 200 \\ \midrule
%  \multirow{4}{*}{\paraphrase{}}& \backtranslation{} & 0.1618$^{\downarrow}$ & 0.1546$^{\downarrow}$ & 0.1602$^{\downarrow}$ & 0.1438$^{\downarrow}$ & 0.2036$^{\downarrow}$ & 0.3045$^{\downarrow}$ & 0.2584$^{\downarrow}$ & 93 \\
%  & \tfiveqqp{} & 0.2201 & 0.2065 & 0.2095 & 0.1962 & 0.2614 & 0.3926$^{\downarrow}$ & 0.3214$^{\downarrow}$ & 105 \\
%  & \wordembedsyn{} & 0.1759$^{\downarrow}$ & 0.1719$^{\downarrow}$ & 0.1902$^{\downarrow}$ & 0.1690$^{\downarrow}$ & 0.2142$^{\downarrow}$ & 0.3245$^{\downarrow}$ & 0.2828$^{\downarrow}$ & 124 \\
%  & \wordnetsyn{} & 0.1791$^{\downarrow}$ & 0.1751$^{\downarrow}$ & 0.1957$^{\downarrow}$ & 0.1765$^{\downarrow}$ & 0.2117$^{\downarrow}$ & 0.3244$^{\downarrow}$ & 0.2733$^{\downarrow}$ & 71 \\ \bottomrule
% \end{tabular}
% \end{table*}

==> tables/uqv_dist.tex <==
\begin{table}
\caption{Distribution of \uqv{} query variations for categories based on the manual annotations of tuples of queries from the same information need. \todo{misspelling is not here because UQV data we used already had fixed misspelling variations. I will see if I can get an estimate of how many misspellings they corrected to add here.}}
\label{table:uqv_dist}
\begin{tabular}{lcc}
\toprule
\textbf{Category} & \textbf{Count (\%)} & \textbf{Changes semantics}\\
\midrule
\genspec{} & 172 (26.34\%) & $\checkmark$ \\
\aspectchange{} & 111 (17.00\%) & $\checkmark$ \\ 
\paraphrase{} & 215 (32.92\%) \\
\naturality{} & 118 (18.07\%) \\
\ordering{} & \phantom{0}37 (\phantom{0}5.67\%) \\ \bottomrule
\end{tabular}
\end{table}

==> tables/valid_by_method.tex <==
\begin{table}[]
\caption{Percentage of valid queries by automatic query variation method based on manual annotation of queries from the test sets.}
\label{table:valid_by_method}
\begin{tabular}{@{}lrr@{}}
\toprule
\textbf{Method name} & \multicolumn{1}{l}{\textbf{\trecdl{}}} & \multicolumn{1}{l}{\textbf{\antique{}}} \\ \midrule
\charswap{} & 100.00\% & 99.50\% \\
\charsub{} & 97.67\% & 91.00\% \\
\charqwerty{} & 97.67\% & 98.50\% \\
\removestop{} & 86.05\% & 99.50\% \\
\tfiverectotitle{} & 81.40\% & 68.00\% \\
\orderswap{} & 100.00\% & 100.00\% \\
\backtranslation{} & 53.49\% & 46.50\% \\
\tfiveqqp{} & 60.47\% & 52.50\% \\
\wordembedsyn{} & 62.79\% & 62.00\% \\
\wordnetsyn{} & 37.21\% & 35.50\% \\ \bottomrule
\end{tabular}
\end{table}
